Interval-valued aggregation functions based on moderate deviations applied to Motor-Imagery-Based Brain Computer Interface

In this work we study the use of moderate deviation functions to measure similarity and dissimilarity among a set of given interval-valued data. To do so, we introduce the notion of interval-valued moderate deviation function and we study in particular those interval-valued moderate deviation functions which preserve the width of the input intervals. Then, we study how to apply these functions to construct interval-valued aggregation functions. We have applied them in the decision making phase of two Motor-Imagery Brain Computer Interface frameworks, obtaining better results than those obtained using other numerical and intervalar aggregations.

==> gallery/fig_acc_binary_task.tex <==
\begin{tabular}{lrr}
\toprule
{} &      trad &       mff \\
\midrule
Kleene-Dienes &  0.741833 &  0.774813 \\
Lukasiewicz   &  0.762484 &  0.758375 \\
Reinchenbach  &  0.741833 &  0.774813 \\
\bottomrule
\end{tabular}


==> gallery/p_values_binary.tex <==
\begin{tabular}{llllll}
\toprule
{} &   OWA1 &   OWA2 &   OWA3 &    MD2 & MD5 \\
\midrule
OWA1 &        &        &        &        &     \\
OWA2 &  \$.25\$ &        &        &        &     \\
OWA3 &  \$.25\$ &  \$.25\$ &        &        &     \\
MD2  &  \$.25\$ &  \$.25\$ &  \$.25\$ &        &     \\
MD5  &  \$.09\$ &  \$.02\$ &  \$.09\$ &  \$.02\$ &     \\
\bottomrule
\end{tabular}

